A Tight VC-Dimension Analysis of Clustering Coresets with Applications

We consider coresets for $k$-clustering problems, where the goal is to assign points to centers minimizing powers of distances. A popular example is the $k$-median objective $\sum_{p}\min_{c\in C}dist(p,C)$. Given a point set $P$, a coreset $\Omega$ is a small weighted subset that approximates the cost of $P$ for all candidate solutions $C$ up to a $(1\pm\varepsilon )$ multiplicative factor. In this paper, we give a sharp VC-dimension based analysis for coreset construction. As a consequence, we obtain improved $k$-median coreset bounds for the following metrics: Coresets of size $\tilde{O}\left(k\varepsilon^{-2}\right)$ for shortest path metrics in planar graphs, improving over the bounds $\tilde{O}\left(k\varepsilon^{-6}\right)$ by [Cohen-Addad, Saulpic, Schwiegelshohn, STOC'21] and $\tilde{O}\left(k^2\varepsilon^{-4}\right)$ by [Braverman, Jiang, Krauthgamer, Wu, SODA'21]. Coresets of size $\tilde{O}\left(kd\ell\varepsilon^{-2}\log m\right)$ for clustering $d$-dimensional polygonal curves of length at most $m$ with curves of length at most $\ell$ with respect to Frechet metrics, improving over the bounds $\tilde{O}\left(k^3d\ell\varepsilon^{-3}\log m\right)$ by [Braverman, Cohen-Addad, Jiang, Krauthgamer, Schwiegelshohn, Toftrup, and Wu, FOCS'22] and $\tilde{O}\left(k^2d\ell\varepsilon^{-2}\log m \log |P|\right)$ by [Conradi, Kolbe, Psarros, Rohde, SoCG'24].

==> sections/06-z-greater-than-one.tex <==
\section{Trying to work out the new stuff}

% \subsection{Chris's email to me}

%%%%%%%%%%%%%%%%%%%% EMAIL TEXT %%%%%%%%%%%%%%%%%%%%%%
% I confused myself. Sorry. I think it works.

% we have a very good alpha-net for type i up to precision alpha > 2^(-i/z) of size exp(k)

% we also have a net for type i of size alpha^-1 * 2^(i/z) * k D

% the overall variance of the estimator is

% k_i / k * k^2 * alpha^2 * 2^(2i(1-1/z)) / (k_i 2^i + k)^2

% where k_i is the number of clusters of type i.

% If you do the caluclations, you get that this is at most alpha^2 * 2^(2i -2i/z)  / 2^i

% which simplifies to alpha * 2^(i - 2i/z)) 

% So when doing the chaining we have

% sum_ 2^h < 2^i/z (something small)  (for the coarse part) 
% and
% sum 2^h > 2^i/z     sqrt(kd 2^h 2^i/z * 2^-2h * 2^(i-2i/z) for the finer part.

% the latter part is now

% sum 2^h > 2^i/z     sqrt(kd 2^-h * 2^(i(z-1)/z))

% since 2^h > 2^i/z, we now get

% sqrt(kd 2^i(z-2)/z) = sqrt(kd 2^(i-2)) as desired

\subsection{Net size}

\andrewfixme{I'm using $\alpha$ for the nets. Otherwise, it is extremely confusing if we use an $\varepsilon$ for the coreset guarantee and a separate $\varepsilon$ for the nets.}
\begin{lemma}
    \andrewfixme{I am not confident about the actual net size in this lemma statement because I'm not sure how the Sauer-Shelah stuff goes through.}
    For any main group $G$, there exists a type $i$ approximate centroid set $\cN_{G}(\alpha, k, 2^i)$ for $G$ of size
    \[
        \left\lvert\cN_{G}\left(\varepsilon, k, r\right)\right\rvert \leq \exp{ { \gamma\cdot k\log k \cdot  \alpha^{-1} 2^{i/z} \log\left( \alpha^{-1} 2^{i/z} \right) \cdot d_{\VC} \cdot \log |G|}},
    \]
\end{lemma}
\begin{proof}
    \andrewfixme{I am guessing as to what the net definition is based on bread crumbs. If this is incorrect, then I'm not sure what I'm doing.}
    Let $p$ be any point belonging to cluster $C$ of type $i$. Recall by the definition of a type $i$ $\alpha$-net $\cN^i_{G}(\alpha, k, 2^i)$ that we are discretizing the space so that, given approximate and candidate solutions $\cA$ and $\cS$, for any cluster in type $i$ we have
    \[ |\cost(p, \tilde \cS) - \cost(p, \cS)| \leq \frac{\alpha}{z\log(z/\alpha)} \cdot \dist^{z-1}(p, \cS) \cdot \dist(p, \cA), \]
    where $\tilde \cS$ is $\cS$'s closest representative in $\cN^i_{G}$. We will construct this net by discretizing the range from the smallest point-center distance in this type to the largest.

    Specifically, define 
    \begin{align*}
        d_{min} &= \min_{p \in C \in T_i} \cost(p, \cS) \\
        d_{max} &= \max_{p \in C \in T_i} \cost(p, \cS).
    \end{align*}
    By the group property, these are within a constant factor of each other. \andrewfixme{A factor $2$, right?} Lastly, we define the following increment size
    \[ I \coloneq \min_{p \in C \in T_i} \dist(p, \cS)^{z-1} \dist(p, \cA). \]

    \noindent Now, define $r_0 = d_{min}$ and let $r_i = r_{i-1} + \alpha I$ be the ranges which go from $d_{min}$ to $d_{max}$ in increments of $\alpha I$. That is, our final index $j$ is where $r_j = r_0 + j \cdot \alpha \cdot I \geq d_{max}$. We now solve for the number of these ranges:
    \begin{align*}
        r_0 + j \cdot \alpha \cdot I &= \dist(p, \cS)^z \\
        &= 2^i \cdot \dist(p, \cA)^z \\
        \rightarrow j &= \frac{2^i \cdot \dist(p, \cA)^z - r_0}{\alpha \cdot I} \\
        &\leq \frac{2^i \cdot \dist(p, \cA)^z}{\alpha \cdot 2^{i(1 - 1/z)} \cdot \dist(p, \cA)^z} \\
        &= \alpha^{-1} \cdot 2^{i/z},
    \end{align*}
    where the inequality is by ignoring $r_0$ and by Lemma \ref{lem:represent_costqS_via_p}.
    
    \andrewfixme{I'm assuming we get from this to nets of size $\exp{\alpha^{-1} \cdot 2^{i/z} \cdot k \cdot d_{vc} \cdot \log(\text{something})}$ by using Sauer-Shelah and VC-dimension stuff? Not 100\% clear to me how this comes together though, since we're not really doing ranges in the traditional sense. I.e., they're not actually with respect to radial balls but with respect to $\dist(p, \cS)^{z-1} \dist(p, \cA)$. Is the VC-dimension of this the same? If yes, it requires a proof.}
\end{proof}

\subsection{Chaining}

We re-write our estimator as
\[ \sum_{C \in T_i} \frac{ \sum_{p \in C} \left( v_p^{\cS, \log \left( 2^{i/z} \right)} -q_0  + q_0 + \sum_{h = \log \left( 2^{i/z} \right)}^{\infty} \left( v_p^{\cS, h+1} - v_p^{\cS, h}\right) \right) \cdot w_p \cdot g_p}{|\Omega| \cdot (\cost(G, \cS) + \cost(G, \cA))}. \]
\andrewfixme{I believe we \emph{need} to have the denominator be of the form $\left(\cost(C, \cS) + \cost(C, \cA)\right)$ rather than $\cost(G, \cS) + \cost(G, \cA)$ if we are going to use type-based inequalities to relate $\cost(\_, \cS)$ to $2^i \cost(\_, \cA)$. Specifically, we don't have a guarantee that the entire group belongs to a type, so we cannot apply this equivalence with respect to the group costs. We also \emph{cannot} do $k \cdot \left(\cost(C, \cS) + \cost(C, \cA)\right)$ in the denominator because $k \cdot \left(\cost(C, \cS) + \cost(C, \cA)\right) \geq \cost(G, \cS) + \cost(G, \cA)$. The consequence is that, when doing the chaining for $v_p^{\cS, h+1} - v_p^{\cS, h}$, there will be a $k$ in the numerator that I cannot make cancel out. The following is the derivation to see where the $k$ comes from that doesn't cancel.} 

\andrewfixme{As a consequence, we need to prove that bounding the variance with respect to this denominator is actually correct with respect to the interactions with the other lemmas.}

\noindent We then separate this into three terms:
\begin{align*}
    \text{Term 1}&: \quad \frac{ \sum_{C \in T_i} \sum_{p \in C} \left( v_p^{\cS, \log \left( 2^{i/z} \right)} -q_0 \right) \cdot w_p \cdot g_p}{|\Omega| (\cost(G, \cS) + \cost(G, \cA))}, \\
    \text{Term 2}&: \quad \frac{\sum_{C \in T_i} \sum_{p \in C} q_0 \cdot w_p \cdot g_p}{|\Omega| (\cost(G, \cS) + \cost(G, \cA))}, \text{ and}\\
    \text{Term 3}&: \quad \frac{\sum_{C \in T_i} \sum_{p \in C} \left(  \sum_{h = \log \left( 2^{i/z} \right)}^{\infty} \left( v_p^{\cS, h+1} - v_p^{\cS, h} \right) \cdot w_p \cdot g_p \right)}{|\Omega| (\cost(G, \cS) + \cost(G, \cA))} \\
    &= \sum_{h = \log \left( 2^{i/z} \right)}^{\infty} \frac{ \sum_{C \in T_i} \sum_{p \in C} \left( v_p^{\cS, h+1} - v_p^{\cS, h} \right) \cdot w_p \cdot g_p }{|\Omega| (\cost(G, \cS) + \cost(G, \cA))}
\end{align*}

\noindent We now want to obtain good variance bounds for each of the three terms using chaining. For each, we can write the variance of the Gaussian variable as
\[ \text{Var}\left[ \sum_{C \in T_i} \sum_{p \in C} \frac{ f(p) \cdot w_p \cdot g_p}{|\Omega| \cdot (\cost(G, \cS) + \cost(G, \cA))} \right]  \leq \sum_{C \in T_i} \sum_{p \in C} \left[ \frac{f(p) \cdot w_p}{|\Omega| \cdot (\cost(G, \cS) + \cost(G, \cA))} \right]^2, \]

\noindent where $f(p)$ represents some function of $p$ which differs between terms $1$, $2$ and $3$. We therefore wish to bound these variances. 

We start with Term 3 for each individual summand of $h$. Here, notice that we can write
\begin{align*}
    |v_p^{\cS, h+1} - v_p^{\cS, h}| &= | v_p^{\cS, h+1} - \dist(p, \cS)^{z-1} \dist(p, \cA) + \dist(p, \cS)^{z-1} \dist(p, \cA) - v_p^{\cS, h} | \\
    &\leq | v_p^{\cS, h+1} - \dist(p, \cS)^{z-1} \dist(p, \cA)| + |\dist(p, \cS)^{z-1} \dist(p, \cA) - v_p^{\cS, h} | \\
    &\leq 2 \cdot 2^{-h} \dist^{z-1}(p, \cS) \dist(p, \cA) \cdot \frac{1}{z \log(z / 2^{-h})} \\
    &\leq \frac{2}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot 2^{i(1 - 1/z)} \cost(p, \cA),
\end{align*}
where the second to last inequality is by the definition of our $\alpha$-net at precision $2^{-h}$ and the last inequality is by Lemma \ref{lem:represent_costqS_via_p}. We also notice that we can write, for $p \in C$,
\begin{align*}
    \cost(p, \cA) \cdot w_p &\leq 2 \frac{\cost(C, \cA)}{|C|} \cdot w_p \\
    &= 2 \frac{\cost(C, \cA)}{|C|} \cdot \frac{\cost(G, \cA) |C|}{\cost(C, \cA)} \\
    &= 2 \cost(G, \cA) \\
    &\leq 4 k' \cdot \cost(C, \cA),
\end{align*}
where $k'$ is the number of clusters in group $G$.

We now plug these both into term 3's variance for a single summand of $h$ to obtain:
\begin{align*}
    \text{Var}[\text{Term 3 at }h] &= \sum_{C \in T_i} \sum_{p \in C} \left( \frac{  \left( v_p^{\cS, h+1} - v_p^{\cS, h} \right) \cdot w_p }{|\Omega| \cdot (\cost(G, \cS) + \cost(G, \cA))}\right)^2 \\
    &\leq \sum_{C \in T_i} \sum_{p \in C} \left( \frac{ \frac{2}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot 2^{i(1 - 1/z)} \cost(p, \cA) \cdot w_p }{|\Omega| \cdot (\cost(G, \cS) + \cost(G, \cA))}\right)^2 \\
    &\leq \sum_{C \in T_i} \sum_{p \in C} \left( \frac{ \frac{8}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot 2^{i(1 - 1/z)} \cdot k \cdot \cost(C, \cA) }{|\Omega| \cdot (\cost(G, \cS) + \cost(G, \cA))}\right)^2 \\
    &\leq \sum_{C \in T_i} \sum_{p \in C} \left( \frac{ \frac{8}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot k' \cdot 2^{i(1 - 1/z)} \cdot \cost(C, \cA) }{|\Omega| \cdot 2^{i} \cost(G, \cA) + \cost(G, \cA)}\right)^2 \\
    % &= \sum_{C \in T_i} \sum_{p \in C} \left( \frac{ \frac{8}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot k \cdot 2^{i(1 - 1/z)}}{|\Omega| \cdot (2^{i} + 1)}\right)^2 \\
    % &\leq \sum_{C \in T_i} \sum_{p \in C} \left( \frac{ \frac{8}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot k \cdot 2^{i(1 - 1/z)}}{|\Omega| \cdot 2^{i}}\right)^2 \\
    % &\leq \sum_{C \in T_i} \sum_{p \in C} \left( \frac{ \frac{8}{z \log(z / 2^{-h})} \cdot 2^{-h} \cdot k \cdot 2^{-i/z}}{|\Omega|}\right)^2 \\
\end{align*}

\andrewfixme{The $k$ in the above is a $k'$}

\andrewfixme{So, in essence, we can make the derivation in the email generally go through but since we can't do the step of $\cost(G, \cS) = 2^i \cdot \cost(G, \cA)$, we can't make it go through perfectly and will need to amend things.}

Chris:

%\sum -> k_i/k' conditioned on event E
%var 2^(2i(1-1/z))

\begin{align*}
    Var &= \frac{1}{\Omega}\cdot
    \alpha^2 \frac{k_i}{k'} \cdot \frac{k'^2 \cdot 2^{2i(1-1/z)}}{(k_i2^i + k')^2} \\
    &=\frac{1}{\Omega}\cdot\alpha^2 k_i \cdot \frac{k' \cdot 2^{2i(1-1/z)}}{k_i2^i k'} \\
    &=\frac{1}{\Omega}\cdot\alpha^2  2^{i(1-2/z)} \\
\end{align*}

Net size: $\exp{k\cdot \alpha^{-1}2^{i/z}}$

$$\alpha = 2^{-h}$$

\begin{align*}
  &\sum_{h> \log 2^{i/z} \Leftrightarrow\alpha <2^{-i/z}} \sqrt{\log|N| \cdot Var} = \sum_{\alpha} \sqrt{k\cdot \alpha^{-1}2^{i/z} \cdot \frac{1}{\Omega}\cdot\alpha^2  2^{i(1-2/z)}} \\
  =&\sum_{\alpha <2^{-i/z}} \sqrt{k \cdot \frac{1}{\Omega}\cdot\alpha  2^{i(1-1/z)}} \\
  =&\sum_{\alpha <1} \sqrt{k \cdot \frac{1}{\Omega}\cdot \alpha 2^{i(1-2/z)}}
\end{align*}
%this converges (geometric series)

% The last step here is that we are multiplying by alpha < 2^{-i/z} so we now sum by \alpha' = \alpha * 2^{-i/z} and then the alpha primes are the summand term. So this is equivalent to doing h starting at 1 going to infinity essentially.

% This is all to give us the (1 - 2/z) in the exponent which will facilitate k-means going through


% We now use the following inequalities:
% \begin{enumerate}
%     \item For any cluster $C$ in group $G$, the group properties give us $\cost(G, \cA) \leq 2 k \cdot \cost(C, \cA)$.
%     \item Similarly, the type properties give us $\cost(C, \cS) \geq 2^i \cdot \cost(C, \cA)$ \andrewfixme{Check the constants on this second inequality! I'm being flippant by just saying $\cost(p, \cS) = 2^i \cost(p, \cA)$!}
% \end{enumerate}

\subsubsection{Chris Explanation}

$\frac{1}{|\Omega|}\sum_{C_j\in T_i} \frac{\sum_{p\in C_j\cap \Omega}q_j g_p}{\text{cost}(G,S)+\text{cost}(G,A)}$.

$$\text{cost}(G,S) \geq \sum_{C_j \cap G}\text{cost}(C_j\cap G,S) = \sum_j b_j$$, then $b_j = \cost(C_j \cap G, \cS)$.

$$\sum \frac{a_j}{\sum b_j}\leq \max \frac{a_j}{b_j}$$

%%%%%%%%%%%%%%%%%%%% EMAIL TEXT %%%%%%%%%%%%%%%%%%%%%%
% I guess there is still a mistake for k-median. Here is an outline for how to make everything work

% 1. you can get an eps net, for type i, of size

% exp(eps^-1 * 2^(i/z) k d)

% proof: 
% consider the points that have distance D in A. (and cost D^z in A)
% in type i, everthing costs between 2^i * D^z and, say, 10 * 2^i * D^z

% further F := (2^i * D)^((z-1)/z) = dist^(z-1) (p,S) 

% increment everything by j * eps * F * D.

% you need j_max > (10 * 2^i * D^z)/eps * F *D 

% solve this, and you get j_max > eps^-1 * 2^(i/z), up to constants.

% Now in the chaining, we write the following.

% Let v be the cost vector, let v^h be the approximation from an eps-net.

% 2. Chaining
% We write
% v = v^(log (2^(-i/z)) - q_0  + q_0 + sum_(h >= log 2^i/z) v^h+1 - v^h    
% q_0 is the minimum cost point in the cluster that p is in; should write it as q(p)

% we have concentration for q_0
% the variance for the steps v^h+1 - v^h (as well as the step v^(log (2^(-i/z)) - q_0)

% is 

% 1/\Omega^2 sum_{p in \Omega \cap Type i}  (cost(G,A)/(cost(G,A) + cost(G,S)) * (2^-h) * F * D)^2.

% cost(G,A) = k (by group property,
% cost(G,S) = k_i * 2^i

% (2^-h * F * D)^2 = 2^-2h * D^(2z) * 2^(2i *(z-1)/z)

% D^2z cancels out, so let's look at what is left. we get

% 1/Omega^2 sum 2^-2h 2^(2i * - 2i/z) * k^2/(k*k_i*2^i)

% conditioned on event E, we have Omega * k_i/k many elements in the sum. Then the variance becomes
% 1/\Omega 2^-2h 2^(i * - 2i/z)

% now look at the union bound. 

% sum_h> log 2^i/z sqrt( k * d * 2^h * 2^i/z * 2^-2h 2^(i * - 2i/z) / \Omega)

% = sum_h> log 2^i/z sqrt( k * d *  2^-h 2^(i * - i/z) / \Omega)

% = sum_h> 0 sqrt( k * d *  2^-h 2^(i * - 2i/z) / \Omega)

% since 2^i < eps^-z, this is at most

% = sum_h> 0 sqrt( k * d *  2^-h eps^(-z+2) / \Omega)

%%%%%%%%%%%%%%%%%%%% Working it out below %%%%%%%%%%%%%%%%%%%%%%





% k' = num clusters in G; we've normalized all of them to cost 1
% k_i is the num clusters of type i
% cost(G, A) = k'
% cost(G, S) \geq k_i * 2^i

% 


==> sections/07-applications.tex <==
\section{Applications}
\label{sec:applications}
We briefly outline a few applications of Theorem \ref{thm:main}. Similar bounds can also be given via Theorem \ref{thm2} for other $(k,z)$ clustering objectives.\\

\noindent\textbf{Minor Free Graphs.}
For $K_h$ minor free graphs, the VC dimension of the range space induced by metric balls with respect to shortest path distances is bounded by at most $h-1$, see \cite{BousquetT15,ChepoiEV07,LeW24}. 
This immediately gives rise to the following corollary.
\begin{corollary}
Given a (potentially weighted) graph $G(V,E)$ excluding a minor of size $h$, there exists a coreset for $k$-median clustering with respect to shortest path distances of size
$$\Tilde{O}(kh \varepsilon^{-2}).$$
\end{corollary}
As mentioned in the introduction, for planar graphs in particular, this yields a coreset whose size is $\Tilde{O}(k \varepsilon^{-2})$, which improves over the $\Tilde{O}\left(k\varepsilon^{-6}\right)$ bound of \citet{Cohen-AddadSS21} and the $\tilde{O}\left(k^2 \varepsilon^{-4}\right)$ bound by \citet{BravermanJKW21}. More generally for minor free (but not necessarily planar) graphs, the previous results by \citet{BravermanJKW21} yields a coreset of size $\tilde{O}\left(k^2 \varepsilon^{-4} \cdot f(h)\right)$, where $f(h)$ is at least doubly exponential in $h$, and by \citet{BravermanCJKST022} yields a coreset of size $\Tilde{O}\left(k^3 h \varepsilon^{-3}\right)$.\\

\noindent\textbf{Polygonal Curves and Frechet Distance.}
Another important set system are metric balls induced by the Frechet distance with respect to polygonal curves. A polygonal curve $P$ of length $m$ is a sequence of vertices $p_1,\ldots p_m \in \mathbb{R}^d$, where consecutive pairs of vertices create edges. Given two curves $P_1$ and $P_2$, a warping path is a sequence $(1,1)=(i_1,j_1),(i_2,j_2),\ldots,(i_M,j_M) = (|P_1|,|P_2|)$ such that $i_k-i_{k-1}$ and $j_k-j_{k-1}$ are either $0$ or $1$ for all $k$. The set of all warping paths between $P_1$ and $P_2$ are denoted by $\mathcal{W}_{P_1,P_2}$.
Then the discrete Frechet distance is defined as
$$\dist_{dF}(P_1,P_2) = \min_{w\in \mathcal{W}_{P_1,P_2}}\max_{(i,j)\in w} \|p_i-q_j\|,$$
where $\|x\| = \sqrt{\sum x_i^2}$ is the Euclidean norm.

In the continuous case, we view a polygonal curve $P:[0,1]\rightarrow \mathbb{R}^d$ by fixing $m$ values $0=t_1<\ldots<t_m=1$ and defining $P(t)=\lambda p_{i+1}- (1-\lambda)p_{i}$ where $\lambda=\frac{t-t_i}{t_{i+1}t_i}$ for $t_i\leq t\leq t_{i+1}$.
The continuous Frechet distance between two curves $P_1$ and $P_2$ is defined as 
$$\dist_{F}(P_1,P_2) = \underset{\alpha,\beta:[0,1]\rightarrow [0,1]}{\text{inf}}\underset{t\in [0,1]}{\text{sup}} \|P_1(\alpha(t))-P_2(\beta(t))\|.$$

In recent work, \citet{BD23} and \citet{ChengH24} showed that if the center curves have length at most $\ell$ and the input curves have length at most $m$, the VC dimension of metric balls for both discrete and continuous Frechet distance may be bounded by $O(d\ell\log(\ell m))$, see also \cite{DriemelNPP21} for earlier, slightly weaker bounds. 
The $(k,\ell)$ clustering problem with respect to the Frechet distance uses at most $k$ centers of length at most $\ell$, while minimizing the sum of Frechet distances. For this problem, we obtain the following result:
\begin{corollary}
Given a set of polygonal curves of length at most $m$, there exists a coreset for $k$ median clustering with respect to the discrete or continuous Frechet distance of size
$$\Tilde{O}(kd\ell \log(m)\varepsilon^{-2}).$$
\end{corollary}
The previous state of the art seems to be a recent result \citet{ConradiKPR24}, giving coresets of size $\Tilde{O}\left(k^2d\ell\varepsilon^{-2}\log m \log n\right)$, or alternatively trading the dependency on $\log n$ with a dependency on $k/\varepsilon$, the $\Tilde{O}\left(k^3d\ell\varepsilon^{-3}\log m \right)$ result by \citet{BravermanCJKST022}.
% For discrete Frechet distances, the dependency on $d$ may be replaced with a dependency on $\varepsilon^{-2}$, for which we briefly sketch the reduction. 
% Given a set of points $P\subset \mathbb{R}^d$, a terminal embedding is a mapping $f:\mathbb{R}^d\rightarrow \mathbb{R}^{d'}$ such that
% $$\forall x\in P,\forall y\in \mathbb{R}^d.~~ \|f(x)-f(y)\| = (1\pm \varepsilon)\cdot \|x-y\|.$$
% A terminal embedding, applied to all vertices of a polygonal curve, preserves its discrete Frechet distance to any other polygonal curve. The target dimension $d'$ required is $O(\varepsilon^{-2}\log |P|)$, i.e. the same target dimension as given by the Johnson-Lindenstrauss lemma, in spite of the stronger guarantee \cite{NarayananN19}.
% Applying a terminal embedding to a set of $n$ polygonal curves of length at most $n$ allows us to replace $d$ with $\varepsilon^{-2}\log(nm)$. Thereafter, the iterative size reduction technique from \citet{BravermanJKW21} used in the proof of Theorem \ref{thm:main} allows us to remove the dependency on $\log n$, giving a coreset of size 
% $$\Tilde{O}(k\ell \log^2(m)\left(\varepsilon^{-4}+\varepsilon^{-2-z}\right)).$$
% Terminal embeddings are not known to preserve the the continuous Frechet distance. The interested reader is referred to \cite{MeintrupMR19,psarros2023random} for more results on dimension reduction for polygonal curves.
\\

\noindent\textbf{Hausdorff Metric.}
Given two sets $X,Y\subseteq \mathbb{R}^d$, the directed Hausdorff distance from $X$ to $Y$ is defined as
$$\dist_{\overrightarrow{H}}(X,Y) = \underset{x\in X}{\text{sup}}\underset{y\in Y}{\text{inf}} \|x-y\|$$
and the Hausdorff distance between $X$ and $Y$ is defined as
$$\dist_{H}(X,Y) = \max\left(\dist_{\overrightarrow{H}}(X,Y),\dist_{\overrightarrow{H}}(Y,X)\right).$$
We consider polygonal regions, that is the border of a set $X$ is a polygonal curve with $p_1=p_m$. The $(k,\ell)$-clustering problem  asks to minimize the distance to the closest region with respect to the Hausdorff distance of at most $k$ candidate center regions where the border of each center region is at most $\ell$.
For this metric, \citet{BD23} showed that the VC dimension is of the order $O(d\ell\log(\ell m))$, which combined with Theorem \ref{thm:main} implies
\begin{corollary}
Given a set of polygonal regions with boundary length at most $m$, there exists a coreset for $(k,\ell)$ clustering with respect to the Hausdorff distance of size
$$\Tilde{O}(kd\ell \log(m)\varepsilon^{-2}).$$
\end{corollary}
While it is likely that results by \cite{BuchinR22,ConradiKPR24} would also yield coresets for this problem, the only stated results we are aware of are due to \citet{BravermanCJKST022} who gave a coreset of size $\Tilde{O}\left(k^3 \varepsilon^{-3} d^2 \ell^2 \log m\right)$. The stated result was obtained via the looser VC-dimension bound by \citet{DriemelNPP21} and using the improved bounds by \citet{BD23}, their coreset size should improve to $\Tilde{O}\left(k^3 \varepsilon^{-3} d \ell \log m\right)$. 

\section{A Brief Remark On An Error in a Previous Version}
We had previously claimed a coreset bound of 
$\tilde{O}\left(k\cdot d_{VC}\cdot \left(\varepsilon^{-2}+\varepsilon^{-z}\right)\right)$
for general $(k,z)$ clustering. For $k$-median clustering, the bounds are identical, but Theorem \ref{thm2} is slightly weaker.
We believe that the aforementioned bound is not obtainable and conjecture that the bounds given in Theorem \ref{thm2} are optimal for a worst-case metric for $\varepsilon^{-1}\ll k$, noting that there exist metrics where a VC-dimension based analysis does not yield an optimal coreset size.

To prevent similar errors, we briefly highlight some misleading and wrong claims we encountered in literature. Given two functions $\mathcal{F}$ and $\mathcal{G}$ with set systems induced by $R_f(i,t) = \{x|f_i(x)\geq t\}$ and $R_g(i,t) = \{x|g_i(x)\geq t\}$, for $f_i\in \mathcal{F}$ and $g_i\in \mathcal{G}$, suppose that the VC dimensions are $d_F$ and $d_G$ respectively. The VC dimension of 
$\mathcal{F}-\mathcal{G}$ with ranges $R(i,j,t)=\{x |f_i(x)-g_j(x)\geq t\}$ does not have bounded VC dimension, even if $d_F$ and $d_G$ are $1$.
To see this, suppose $\mathcal{F}$ and $\mathcal{G}$ are defined on the positive integers. Let $\mathcal{A}$ be the set of all functions mapping the positive integers to $\{0,1\}$ and let $\mathcal{F}$ consists of the functions of $2x + a_i(x)$, where $a_i\in \mathcal{A}$. Let $\mathcal{G}$ consist only of the function $2x$. Since $\mathcal{F}$ and $\mathcal{G}$ act monotonously on the positive integers, they have VC dimension $1$. However, $\mathcal{F}-\mathcal{G}$ yields $\mathcal{A}$, which contains the indicator function for every set of positive integers and thus can shatter any set of positive integers.

\section{Funding Acknowledgements}
Andrew Draganov and Chris Schwiegelshohn are partially supported by the Independent Research Fund Denmark (DFF) under a Sapere Aude Research Leader grant No 1051-00106B. Matteo Russo is partially supported by the ERC Advanced Grant 788893 AMDROMA ``Algorithmic and Mechanism Design Research in Online Markets'', by the FAIR (Future Artificial Intelligence Research) project PE0000013, funded by the NextGenerationEU program within the PNRR-PE-AI scheme (M4C2, investment 1.3, line on Artificial Intelligence), by the PNRR MUR project IR0000013-SoBigData.it, and by the MUR PRIN grant 2022EKNE5K (Learning in Markets
and Society). 

==> sections/old.tex <==
% What remains is to give the space bound. The number of points added to the coreset due to Lemma \ref{lem:nets2coresets-inner} is at most $O(k \log^3 k\varepsilon^{-1})$, so we focus on the other groups.
% Setting $m$ initially to 
% \newline
% $O\left(kd \left(\varepsilon^{-2}+\varepsilon^{-z}\right)\text{polylog}(k\varepsilon^{-1})\log^2 n \log 1/\delta\right)$ ensures that the bounds in \ref{lem:nets2coresets}, \ref{lem:nets2coresets-outer} hold with probability $1-\delta$. Recursively applying the coreset construction on the initial coreset once ensures that we have a coreset with multiplicative error $(1\pm \varepsilon)$ with probability $1-\delta$ and with $$m\in O\left(kd \left(\varepsilon^{-2}+\varepsilon^{-z}\right)\text{polylog}(k\varepsilon^{-1})\log^2\log n \log 1/\delta\right).$$
% We now use the iterative size reduction given by Theorem 3.1 from \citet{BravermanJKW21}. Specifically, the theorem states that, given a set of points $P$, any coreset algorithm of size $T\cdot \varepsilon^{-c} \log |P| \log 1/\delta$ succeeding with probability $1-\delta$ can be used iteratively to yield a coreset of size $O\left(T\cdot \varepsilon^{-c} \log \frac{T}{\varepsilon} \log 1/\delta\right)$ succeeding with probability $1-\delta$ in polynomial time, if $|P|$ is the distinct number of points and $c$ is an absolute constant.\footnote{One needs to be careful that the dependency on $\log n$ is indeed the distinct number of points, and not related to the overall weight of the points. In particular, the latter is true for Chen's algorithm \cite{Chen09}, which is why the $\log n$ dependency cannot be removed from said construction. In the context of our analysis, $\log n$ is the distinct number of points and thus the iterative size reduction can be used. We remark that the iterative size reduction is not necessary and the coreset can be computed in one shot, by way of making the nets only dependent on the sample. This is not a new technique, having been used in \cite{BCPSS24,Cohen-AddadLSSS22,Huang0024}, but requires additional steps in the analysis. For the sake of brevity, we gave the shortest proof.}  
% Since $\log^2 \log n\in O(\log n)$, the theorem follows after a suitable rescaling of $\varepsilon$.

% Lemma \ref{lem:nets2coresets-inner} is very simple to prove, merely using that an inner group $G$ is very cheap and can be summarized by the centers of $\cA$ weighted by the number of points in the intersection of the respective clusters and $G$.
% The main difficulty is to prove Lemmas \ref{lem:nets2coresets} and \ref{lem:nets2coresets-outer}.
% Since we are using sampling to estimate the cost in both cases, we require a bound on the variance of the estimators, as well as a bound on the number solutions in the approximate centroid set. For the variance, previous work gave tight bounds. We therefore focus on the enumeration over solutions, which has been the bottleneck of previous works.
% We first do this in the following section for main groups, followed by a proof of Lemma \ref{lem:nets2coresets}.

%%%%%%%%%%%%%

% The next claim establishes an equivalence between the concept of approximate centroid set and that of a clustering net. \changed{\textbf{QUESTION FOR CHRIS}: why do we even have both clustering nets and approximate centroid sets as different things? We only use clustering nets in all the proofs and we never really care about the explicit approximate centroid set solution in this paper. Can we just do away with the approximate centroid sets entirely?}

% \begin{claim}\label{cl:nets2apx}
% For any point set $P$, there exists a type \changed{i clustering net $\cN_P(\alpha, 2^{i+1})$ of size $N$ if there exists a type $i$ approximate centroid set $\cN_P(\alpha, 2^{i+1})$ of size $N$.} Moreover, there exists a type \changed{$i$ approximate centroid set $\cN_P(\alpha, 2^{i+1})$ of size $N$ if there exists a type $i$ $\cN_P(\alpha/2, 2^{i+1})$ clustering net of size $N$.} 
% \end{claim}
% \begin{proof}
%     \changed{The first implication follows by definition: We simply let $v$ be the cost vector induced by the solution $\Tilde{S}$ from the approximate centroid set. For the second claim, consider any two solutions $\cS',\cS$ for which $v$ satisfies the properties of Definition \ref{def:nets}. Then, for a type $i$ clustering net, 
%     \begin{align*}
%         |\cost(p,\cS') - \cost(p, \cS)| &\leq |\cost(p,\cS') - v_p| + |v_p-\cost(p, \cS)|\\ &\leq 2\alpha \cdot \left( \dist(p, \cS)^{z-1} \cdot \dist(p, \cA) + \dist^z(p, \cS) \right),
%     \end{align*}
%     where the second inequality holds by the definition of clustering nets (and since $\cost(p, \cS) = \dist^z(p, \cS)$). Therefore, we consider the approximate centroid set that contains, for each cost vector $v$, a single representative $\cS$ that satisfies Definition \ref{def:nets} with $v$, which concludes the proof.}
% \end{proof}

%%%%%%%%%%%%%%%%%

% \begin{proof}
% Let us begin by considering the case of a single center, i.e., $I_j=1$. We first illustrate why focusing on the case $z=1$ is without loss of generality. To this end, we provide a one-to-one correspondence between a single center $c$ clustering net for $z=1$ and that for $z > 1$. In particular, consider any point set $X$, and an $\cN_X(\xi^z, 1, 1)$-clustering net for range space $R(c,r,1) = \{p\in X: \dist(p,c)\geq r\}$. Consider the range space $R(c,r,z) = \{p\in X: \dist(p,c)\geq \sqrt[z]{r}\} = \{p\in X: \cost(p,c)\geq r\}$. Then, the $\cN_X(\xi^z, 1, 1)$-clustering net becomes $\cN_X(\xi, 1, z)$-clustering net for $R(c,r,z)$, since $R(c,r,1)$ and $R(c,r,z)$ are completely equivalent.

% We now proceed by rescaling our metric space so that $\cost(p, \cS) \leq r \cdot \cost(p,\cA)\leq 1$ for all $p \in P$, which is without loss of generality. Then, a $\mathcal{N}_{A_j}\left(\left(\frac{\varepsilon}{4z}\right)^z,1,1\right)$-clustering net is contained in a $\mathcal{N}_{A_j}\left(\left(\frac{\varepsilon}{4z}\right)^z,\|.\|_{\infty}\right)$-net with respect to the cost functions induced by a single center \cs{why?}.
% This means that, by Fact~\ref{fct:fat-shattering}, we know that there exists an $\cN_{A_j}(\varepsilon, 1, 1)$-clustering net of size \david{$d_\VC$ of what family?}
% \[
%     |\cN_{A_j}(\varepsilon, 1, 1)| \leq \exp{2d_{\VC}(\gamma_0\varepsilon) \cdot \log |G| \cdot \log\left(\frac{\gamma_1|G|}{ \varepsilon \cdot d_{\VC}(\gamma_0\varepsilon)}\right)},
% \]
% for some universal constants $\gamma_0, \gamma_1$. Moreover, we know that the fat-shattering dimension is upper bounded by the VC dimension \david{VC dim of what ?? a set of real valued function does not have VC dim}, and hence, the above net size can be further upper bounded by 
% \[
%     |\cN_{A_j}(\varepsilon, 1, 1)| \leq \exp{2d_{\VC} \cdot \log |G| \cdot \log\left(\frac{\gamma_1|G|}{ \varepsilon \cdot d_{\VC}}\right)}.
% \]
% To conclude the proof for one single center, we must argue why the above also holds for an clustering net. This follows by the equivalence between clustering nets and clustering nets in Claim~\ref{cl:nets2apx}. 

% Lastly, to extend the above multiple centers, let us just select $I_j$ points from the clustering net. The net size is upper bounded by
% \[
%     |\cN_{A_j}(\varepsilon, I_j, 1)| \leq \exp{2I_j \cdot d_{\VC} \cdot \log |G| \cdot \log\left(\frac{\gamma_1|G|}{ \varepsilon \cdot d_{\VC}}\right)}.
% \]
% This concludes the proof.
% % {\color{red} \begin{itemize}
% %     \item Start with $z=1$. To extend it to $z>1$, we show that a $\mathcal{N}_G(\xi^z,1,1)$-net is a $\mathcal{N}_G(\xi,1,z)$-net, because $R(c,r,1) = \{p\in G ~s.t.~ \dist(p,c)\geq r\}$, $R(c,r,z) = \{p\in G ~s.t.~ \dist(p,c)\geq \sqrt[z]{r}\} = \{p\in G ~s.t.~ \cost(p,c)\geq r\}$. So we can focus on $z=1$.
% %     \item Rescale everything so that our clustering nets are infinity sets. Use the equivalence (Claim 4.2)
% %     \item Invoke the bound on $g_{\infty}$ nets, first by way of Fat shattering, then upper bounding the FSD with the VC dimension (cite these things)
% %     \item We have the claim for one center. Now select $I_j$ points from the clustering net, rather than just $1$.
% % \end{itemize}}
% \end{proof}

==> settings/environments.tex <==
%%%%ENVIRONMENTS%%%%

\theoremstyle{theorem}

\newtheorem{theorem}{Theorem}[section]
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{idea}[theorem]{Idea}

\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}[theorem]{Example}

==> settings/macros.tex <==
%%%%MACROS%%%%

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cZ}{\mathcal{Z}}

\renewcommand{\L}{\textup{L}}
\newcommand{\SW}{\textup{SW}}
\newcommand{\incr}{\textup{incr}}
\newcommand{\dist}{\textup{dist}}
\newcommand{\largeg}{\textup{large}}
\newcommand{\smallg}{\textup{small}}

\newcommand{\Pb}[1]{\mathbb{P}\left[#1\right]}

\newcommand{\R}{\mathbb{R}}
\DeclareMathOperator*{\argmax}{arg\,max}

\newcommand{\E}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\B}{\mathbb{B}}
\renewcommand{\P}[2]{{\mathbb{P}}_{#1}\left[#2\right]}
\renewcommand{\exp}[1]{{\textup{exp}}\left(#1\right)}
\renewcommand{\H}[2]{{\mathbb{H}}\left(#1 \mid #2\right)}
\newcommand{\Bern}[1]{{\textup{Bernoulli}}\left(#1\right)}
\newcommand{\I}[2]{{\mathbb{I}}\left(#1 \mid #2\right)}
\newcommand{\p}[2]{{p}\left(#1 \mid #2\right)}
\newcommand{\tp}[1]{\widetilde{p}\left(#1\right)}
\newcommand{\ind}[1]{\mathbbm{1}\left\{#1\right\}}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\indep}{\perp\kern-5pt\perp}
\renewcommand{\d}{\text{d}}
\newcommand{\V}[2]{\mathbb{V}_{#1}\left[#2\right]}

\newcommand{\alg}{\cA}
\newcommand{\cost}{\textmd{\textup{cost}}}
\newcommand{\ERM}{\textmd{\textup{ERM}}}
\newcommand{\UCBone}{\textmd{\textup{UCB1}}}
\newcommand{\UCB}{\textmd{\textup{UCB}}}
\newcommand{\VC}{\textmd{\textup{VC}}}
\newcommand{\LDim}{\textmd{\textup{LDim}}}
\newcommand{\poly}{\textmd{\textup{poly}}}
\newcommand{\Ber}[1]{\textmd{\textup{Ber}}\left(#1\right)}

\newcommand{\bA}{\textbf{A}}
\newcommand{\bB}{\textbf{B}}
\newcommand{\bC}{\textbf{C}}
\newcommand{\bK}{\textbf{K}}
\newcommand{\bQ}{\textbf{Q}}
\newcommand{\bS}{\textbf{S}}
\newcommand{\bT}{\textbf{T}}
\newcommand{\bU}{\textbf{U}}
\newcommand{\bV}{\textbf{V}}
\newcommand{\bX}{\textbf{X}}
\newcommand{\bY}{\textbf{Y}}
\newcommand{\bW}{\textbf{W}}
\newcommand{\bZ}{\textbf{Z}}
\newcommand{\bb}{\textbf{b}}
\newcommand{\bc}{\textbf{c}}
\newcommand{\be}{\textbf{e}}
\renewcommand{\bf}{\textbf{f}}
\newcommand{\bl}{\textbf{\ell}}
\newcommand{\bp}{\textbf{p}}
\newcommand{\bq}{\textbf{q}}
\newcommand{\br}{\textbf{r}}
\newcommand{\bs}{\textbf{s}}
\newcommand{\bt}{\textbf{t}}
\newcommand{\bv}{\textbf{v}}
\newcommand{\bx}{\textbf{x}}
\newcommand{\by}{\textbf{y}}
\newcommand{\bz}{\textbf{z}}
\newcommand{\balpha}{\textbf{\alpha}}
\newcommand{\bbeta}{\textbf{\beta}}
\newcommand{\blambda}{\textbf{\lambda}}
\newcommand{\bdelta}{\textbf{\delta}}
\newcommand{\beps}{\textbf{\varepsilon}}

\newcommand{\bzero}{\textbf{0}}
\newcommand{\bone}{\textbf{1}}

\newcommand{\barmu}{\overline{\mu}}
\newcommand{\barl}{\overline{\ell}}
\newcommand{\hatl}{\hat{\ell}}

\newcommand\cs[1]{\textcolor{red}{[CS: #1]}}
\newcommand\pd[1]{\textcolor{magenta}{[PD: #1]}}
\newcommand\ff[1]{\textcolor{violet}{[FS: #1]}}
\newcommand\david[1]{\textcolor{orange}{[David: #1]}}
\newcommand\mr[1]{\textcolor{blue}{[Matteo: #1]}}
\newcommand\andrew[1]{{\leavevmode\color{violet}[Andrew: #1]}}
\newcommand\andrewinline[1]{{\leavevmode\color{violet}#1}}
\newcommand\changed[1]{{\leavevmode\color{violet}#1}}
\newcommand\andrewfixme[1]{{\leavevmode\color{violet}[<\textbf{FIXME}> #1 </\textbf{FIXME}>]}}



\newcommand{\inst}{\mathcal{I}}
\newcommand{\eqdef}{\overset{\mathrm{def}}{=\mathrel{\mkern-3mu}=}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{\node[shape=circle,draw,inner sep=2pt] (char) {#1};}}


==> settings/packages.tex <==
%%%%PACKAGES%%%%

\usepackage[margin=1in]{geometry}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[tbtags]{amsmath}
\allowdisplaybreaks
\usepackage{amssymb,amsthm,mathtools, bbm}
\usepackage{physics}
\usepackage{hyperref}
\usepackage[svgnames]{xcolor}
\usepackage[capitalise,nameinlink]{cleveref}
\definecolor{links}{RGB}{11, 85, 255}
\definecolor{cites}{RGB}{0, 200, 0}
\definecolor{urls}{RGB}{255, 116, 0}
\hypersetup{colorlinks={true},linkcolor={links},citecolor=[named]{cites},urlcolor={urls}}
\usepackage[numbers,compress]{natbib}
\bibliographystyle{abbrvnat}
\usepackage{doi}
\usepackage{tikz} 
\usepackage{pgfplots}
\pgfplotsset{compat=1.14}
\usepgfplotslibrary{fillbetween}
\usepackage{hyphenat}
\usepackage[font=footnotesize]{caption}
\usepackage{subcaption}
\usepackage{appendix}
\usepackage{nicefrac}
\usepackage{tcolorbox}
\usepackage{ bbold }
\usepackage{multirow}

\usepackage{todonotes}

\usepackage{thm-restate}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
